Tightly Integrated Motion Classification and State Estimation in Foot-Mounted Navigation Systems

A framework for tightly integrated motion mode classification and state estimation in motion-constrained inertial navigation systems is presented. The framework uses a jump Markov model to describe the navigation system's motion mode and navigation state dynamics with a single model. A bank of Kalman filters is then used for joint inference of the navigation state and the motion mode. A method for learning unknown parameters in the jump Markov model, such as the motion mode transition probabilities, is also presented. The application of the proposed framework is illustrated via two examples. The first example is a foot-mounted navigation system that adapts its behavior to different gait speeds. The second example is a foot-mounted navigation system that detects when the user walks on flat ground and locks the vertical position estimate accordingly. Both examples show that the proposed framework provides significantly better position accuracy than a standard zero-velocity aided inertial navigation system. More importantly, the examples show that the proposed framework provides a theoretically well-grounded approach for developing new motion-constrained inertial navigation systems that can learn different motion patterns.

==> tree.tex <==

\tikzstyle{level 1}=[level distance=3.5cm, sibling distance=3.5cm]
\tikzstyle{level 2}=[level distance=3.5cm, sibling distance=3.5cm]
\tikzstyle{level 3}=[level distance=3.5cm, sibling distance=3cm]
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [rectangle, draw=none, minimum width=3pt, inner sep=0pt]
\tikzstyle{ans} = [color=black]

\begin{figure}
  \centering
   \hrule
   \vspace{2mm}
\begin{tikzpicture}[level distance=3.6cm,
level 1/.style={sibling distance=3.6cm},
level 2/.style={sibling distance=1.2cm},
level 3/.style={level distance = 2cm},grow'=right]
\tikzstyle{every node}=[]
    \node (Root) [text width=1.5cm, align=center,font=\small,rectangle,draw] {Initial state estimates}
        child [] {
        node [text width=0.6cm, align=center, font=\small,rectangle,draw]{$\hat{x}^{\delta^1_1}_{1|1}$\\[0.2em]$P^{\delta^1_1}_{1|1}$\\[0.2em]$w^1_1$}
        child { node [text width=0.6cm, align=center, font=\small,rectangle,draw]{$\hat{x}^{\delta^1_{1:2}}_{2|2}$\\[0.2em]$P^{\delta^1_{1:2}}_{2|2}$\\[0.2em]$w^1_2$}
        node[above left=10pt, draw,fill=gray!50,rounded corners=2pt]{\small KF}
        edge from parent
        node[above,rotate=19, align=center, font=\scriptsize] {$p(\delta_2=1|\delta_1=1)$}
        }
        child [red, dashed] { node [font=\scriptsize] {Removed}
        }
        child [black] { node [text width=0.6cm, align=center, font=\small,rectangle,draw]{$\hat{x}^{\delta^2_{1:2}}_{2|2}$\\[0.2em]$P^{\delta^2_{1:2}}_{2|2}$\\[0.2em]$w^2_2$}
        node[above left=10pt, draw,fill=gray!50,rounded corners=2pt]{\small KF}
        edge from parent
        node[below,rotate=-19, align=center, font=\scriptsize] {$p(\delta_2=3|\delta_1=1)$}
        }
        edge from parent
        node[above,rotate=45,font=\scriptsize, align=center] {$p(\delta_1=1|\delta_0=1)$}
    }
    child {
        node [text width=0.6cm, align=center, font=\small,rectangle,draw]{$\hat{x}^{\delta^2_1}_{1|1}$\\[0.2em]$P^{\delta^2_1}_{1|1}$\\[0.2em]$w^2_1$}
        child [red, dashed] { node [font=\scriptsize] {Removed}
        }
        child [red, dashed] { node [font=\scriptsize] {Removed}
        }
        child { node [text width=0.6cm, align=center, font=\small,rectangle,draw]{$\hat{x}^{\delta^3_{1:2}}_{2|2}$\\[0.2em]$P^{\delta^3_{1:2}}_{2|2}$\\[0.2em]$w^3_2$}
        node[above left=10pt, draw,fill=gray!50,rounded corners=2pt]{\small KF}
        edge from parent
        node[below,rotate=-19, align=center, font=\scriptsize] {$p(\delta_2=3|\delta_1=2)$}
        }
        edge from parent
        node[above, align=center, font=\scriptsize] {$p(\delta_1=2|\delta_0=1)$}
    }
    child {
         node [text width=0.6cm, align=center, font=\small,rectangle,draw]{$\hat{x}^{\delta^3_1}_{1|1}$\\[0.2em]$P^{\delta^3_1}_{1|1}$\\[0.2em]$w^3_1$}
        child [red, dashed] { node [font=\scriptsize] {Removed}
        }
        child [red, dashed] { node [font=\scriptsize] {Removed}
        }
        child [red, dashed] { node [font=\scriptsize] {Removed}
        }
        edge from parent
        node[below,rotate=-45,font=\scriptsize, align=center] {$p(\delta_1=3|\delta_0=1)$}
    };
   % How I'm applying labels to each level.
  % Need to be able to dynamically align nodes at top level
\begin{scope}[every node/.style={text width=1cm, align=center, anchor=center, font=\small,}]
 \node[above=0.3cm of Root-1-1] (labels-level) {$k=2$};
 \node[at =(labels-level-|Root-1)] {$k=1$};
 \node[at =(labels-level-|Root)] {$k=0$};
\end{scope}
\end{tikzpicture}
   \hrule
  \caption{Illustration of the tree structure representation of the Kalman filter bank used to calculate $p(x_{1:k}|y_{1:k})$. To keep a fixed computational complexity the tree is pruned, by removing the least likely branches, to a fixed number of leaves (3 leaves in the illustration) at each time step.}\label{fig:tree}
\end{figure}


